Monojet searches for momentum-dependent dark matter interactions

We consider minimal dark matter scenarios featuring momentum-dependent couplings of the dark sector to the Standard Model. We derive constraints from existing LHC searches in the monojet channel, estimate the future LHC sensitivity for an integrated luminosity of 300 fb$^{-1}$, and compare with models exhibiting conventional momentum-independent interactions with the dark sector. In addition to being well motivated by (composite) pseudo-Goldstone dark matter scenarios, momentum-dependent couplings are interesting as they weaken direct detection constraints. For a specific dark matter mass, the LHC turns out to be sensitive to smaller signal cross-sections in the momentum-dependent case, by virtue of the harder jet transverse-momentum distribution.

==> 4-conclusionsOLD.tex <==


\label{sec:conclusion}

Momentum-dependent couplings between the dark matter and the Standard Model are well-motivated both from a theoretical and a phenomenological perspective. 
Indeed, broad classes of ultraviolet-complete dark matter models predict effective derivative operators at low energy, in particular whenever the dark matter particle is an approximate Goldstone boson
of the underlying theory. This is quite natural in the context of composite Higgs models for the electroweak symmetry breaking. 
%as a consequence of the shift symmetry of pNGBs. 
On the phenomenological side, scenarios involving momentum-dependent couplings can reproduce the observed dark matter abundance in the Universe, while evading the stringent bounds from direct detection experiments.

Monojet searches at the LHC are important probes of dark matter signals. Assuming simple patterns for the dark matter interactions with the Standard Model, we considered two types of couplings exhibiting momentum-dependent or momentum-independent Lorentz structures within an effective field theory framework. The high-energy tails of the monojet differential distributions being harder in the former case, momentum-dependent couplings are expected to be more efficiently constrained by current LHC data. We demonstrated this by studying the monojet search cross section upper limits for the two scenarios based on early 13 TeV LHC data and showed that the cross sections probed assuming momentum-dependent couplings are indeed smaller than their momentum-independent counterparts. We moreover estimated the reach of the LHC assuming an integrated luminosity of 300 fb$^{-1}$ in proton-proton collisions at a center-of-mass energy of 13 TeV. We then applied these results to the model parameter space and compared the ensuing limits to the bound coming from the requirement of not exceeding the observed dark matter abundance in the Universe, while highlighting the corresponding parameter values for which our effective description breaks down based on perturbative unitarity arguments.

Our results show that a good fraction of the parameter space is already excluded by the LHC null results and that a significant portion of it will be covered in the future. An interesting complementarity arises between collider and cosmological observations, as in the region of parameter space under consideration ($m_\eta > m_s/2$) the former tend to probe underabundant dark matter candidates while the latter exclude overabundant ones (assuming a standard cosmological thermal history). Moreover, the differences in the monojet $p_T$ distribution between the two scenarios could provide handles in order to extract information on the nature of the dark matter couplings to the Standard Model. We intend to address this question in a forthcoming publication.


